Automating Code Review: A Systematic Literature Review

Code Review consists in assessing the code written by teammates with the goal of increasing code quality. Empirical studies documented the benefits brought by such a practice that, however, has its cost to pay in terms of developers' time. For this reason, researchers have proposed techniques and tools to automate code review tasks such as the reviewers selection (i.e., identifying suitable reviewers for a given code change) or the actual review of a given change (i.e., recommending improvements to the contributor as a human reviewer would do). Given the substantial amount of papers recently published on the topic, it may be challenging for researchers and practitioners to get a complete overview of the state-of-the-art. We present a systematic literature review (SLR) featuring 119 papers concerning the automation of code review tasks. We provide: (i) a categorization of the code review tasks automated in the literature; (ii) an overview of the under-the-hood techniques used for the automation, including the datasets used for training data-driven techniques; (iii) publicly available techniques and datasets used for their evaluation, with a description of the evaluation metrics usually adopted for each task. The SLR is concluded by a discussion of the current limitations of the state-of-the-art, with insights for future research directions.

==> tables/rq3_table.tex <==
%!TEX root = ../main.tex

\begin{table}
\centering
\caption{Code review tasks for which automated solutions have been proposed\vspace{-0.3cm}}
\label{tab:rq3_training}
    {\scriptsize
   \begin{tabular}{ p{8cm} | p{0.5cm}| p{0.5cm} | p{3.1cm} | p{0.9cm}}
    \rulec
  \multirow{2}{*}{\bf Task} &\multicolumn{2}{c|}{\bf  Test Set Size} &\multirow{2}{*}{\bf Granularity} &  {\bf Approach} \\\cline{2-3}
                                        &       min             &            max              &                                                &  {\bf Deployed} \\ \rulec

    
     %ASSESSING REVIEW QUALITY ---------------------------------------------------------------------------|
      \multicolumn{5}{c}{\bf  Assessing Review Quality} \\ \rulec
     
      Assessing Review Quality through Biometrics (2) 
     & 84
     & 149 
     & code regions, code review 
     & \xmark \\
     
     \cellcolor{lightlightgrey}Classifying the Usefulness of Review Comments (4) 
     &\cellcolor{lightlightgrey} 200 
     &\cellcolor{lightlightgrey} 1.5k 
     &\cellcolor{lightlightgrey} review comment 
     &\cellcolor{lightlightgrey} 2/3\\ 
     
     Identifying/Improving Review Comments Needing Further Explanations(2) 
     & 90
     & 744
     & review comment
     & \xmark\\ 
     \rulec
    
    % CODE CHANGE ANALYSIS ---------------------------------------------------------------------------|
    \multicolumn{5}{c}{\bf Code Change Analysis} \\ \rulec

     \cellcolor{lightlightgrey}Decomposing Tangled Commit (3)
     &\cellcolor{lightlightgrey} 50 
     &\cellcolor{lightlightgrey} 1k 
     &\cellcolor{lightlightgrey} commit 
     &\cellcolor{lightlightgrey} \xmark\\  
     
     Impact Analysis for Code Review (1)
     & -
     & 8.8k
     & PR
     &  \\  
     
     \cellcolor{lightlightgrey}Linking Similar Contributions (2) 
     &\cellcolor{lightlightgrey} 7k 
     &\cellcolor{lightlightgrey} 383k 
     &\cellcolor{lightlightgrey} code change, PR 
     &\cellcolor{lightlightgrey} \xmark\\ 
     
    Predicting Salient-Class (1)
    & - 
    & 7.6k
    & commit
    & \xmark\\
    \rulec

     
     % CODE CHANGE CLASSIFICATION ---------------------------------------------------------------------------|
    \multicolumn{5}{c}{\bf Code Change Classification} \\ \rulec
      
     \cellcolor{lightlightgrey}Identifying Impactful Code Changes (2)
     &\cellcolor{lightlightgrey} 0
     &\cellcolor{lightlightgrey} 21.4k
     &\cellcolor{lightlightgrey} commit
     &\cellcolor{lightlightgrey} 1/2\\
     % end row
    
    Identifying Large-review-effort Code Changes (1) 
     & - 
     & 136k 
     & commit
     & 1/1\\

    \cellcolor{lightlightgrey}Identifying Quickly Reviewable Changes (1) 
     &\cellcolor{lightlightgrey} -
     &\cellcolor{lightlightgrey} 100k
     &\cellcolor{lightlightgrey} PR
     &\cellcolor{lightlightgrey} \xmark\\ 
     
     Predicting Code Changes Approval, Merge, or Need for review (11) 
    & 10k
    & 661.4k
    & diff hunk, method, PR
    & \xmark \\
    \rulec

       % CODE CHANGE QUALITY CHECK ---------------------------------------------------------------------------|
     \multicolumn{5}{c}{\bf Code Change Quality Check} \\ \rulec
     
     \cellcolor{lightlightgrey}Checking Design Patterns Consistency (1) 
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} 68 
     &\cellcolor{lightlightgrey} file 
     &\cellcolor{lightlightgrey}\xmark \\
     
      Generating Review Comments (11) 
     & 2k 
     & 134k 
     & code change, diff hunk, method
     & \xmark \\
     
     \cellcolor{lightlightgrey}Identifying Clone Refactoring Opportunities (1) 
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} 1258 
     &\cellcolor{lightlightgrey} PR 
     &\cellcolor{lightlightgrey} \xmark \\
     
      Predicting Code Defectiveness (2) 
     & 1370 
     & 4.7k
     & file, PR
     & 1/2 \\

    \cellcolor{lightlightgrey}Predicting Problematic Code Elements (3) 
     &\cellcolor{lightlightgrey} 2k 
     &\cellcolor{lightlightgrey} 1M
     &\cellcolor{lightlightgrey} code line, file, PR
     &\cellcolor{lightlightgrey} \xmark \\
     
     Reviewing Code Formatting Violations (1)
     & - 
     & 663k
     & file 
     & \xmark \\ 
     
     \cellcolor{lightlightgrey}Reviewing via Static Analysis (1) 
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} 8.7k 
     &\cellcolor{lightlightgrey} PR
     &\cellcolor{lightlightgrey} 1/1 \\
     \rulec

   % CODE REVIEW SENTIMENT ANALYIS ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Code Review Sentiment Analysis} \\ \rulec
     
      Classifying the Sentiment of Review Comments (1) 
     & - 
     & 1.6k 
     & review comment 
     & \xmark \\
     
    \cellcolor{lightlightgrey}Identifying “Pushback” Feelings in Reviews (1) 
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} ? 
     &\cellcolor{lightlightgrey} code review
     &\cellcolor{lightlightgrey} \xmark\\ 
     
     Identifying Toxic/Uncivil Code Review Comments (4)
     & 3.6k 
     & 19.6k
     & email, review comment, sentence
     & \xmark\\  
     
     \cellcolor{lightlightgrey}Rephrasing Toxic/Uncivil Comments (1)
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} 2.2k 
     &\cellcolor{lightlightgrey} review comment
     &\cellcolor{lightlightgrey} \xmark\\ 
     \rulec
     
        % RETRIVIAL OF SIMILAR CR/CC ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Retrieval of Similar CR/CC} \\ \rulec
     
      Augmenting Reviews (8)
     & 200 
     & 150k 
     & code change, code review, code snippet, diff hunk, review comment
     & 1/8 \\
     
     \cellcolor{lightlightgrey}Mining Code Improvement Patterns (1) 
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} 61.7k 
     &\cellcolor{lightlightgrey} diff hunk 
     &\cellcolor{lightlightgrey} \xmark \\ 
     \rulec
     
     % REVISED CODE GENERATION ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Revised Code Generation} \\ \rulec

     Implementing the Code Change Requested by a Reviewer (11) 
     & 1.7k 
     & 35.6k 
     & code change, diff hunk, method, review comment
     & 1/11 \\
          
      \cellcolor{lightlightgrey}Predicting the Code Output of the Review Process (4) 
     &\cellcolor{lightlightgrey} 1.7k 
     &\cellcolor{lightlightgrey} 16.8k 
     &\cellcolor{lightlightgrey} method
     &\cellcolor{lightlightgrey} \xmark \\
      \rulec
     
      % TIME MANAGEMENT ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Time Management} \\ \rulec
   
    Identifying Blocking Actors in Pull Requests (1)
     & - 
     & 2.9k 
     & PR 
     & 1/1 \\
   
     \cellcolor{lightlightgrey}Predicting Pull Request/Code Review Completion Time (5)
     &\cellcolor{lightlightgrey} 2.9k 
     &\cellcolor{lightlightgrey} 2.9k 
     &\cellcolor{lightlightgrey} code change, commit, PR 
     &\cellcolor{lightlightgrey} 2/2 \\
     
     Prioritizing Review Requests (3)
     & 2.9k
     & 661k
     & code change, PR 
     & 2/5 \\ 
     \rulec
     
      % OTHER ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Other} \\ \rulec
   
     \cellcolor{lightlightgrey}Classifying the Goal of a Review Comment or the Type of Change Triggered by a Comment (3)
     &\cellcolor{lightlightgrey} 1.5k 
     &\cellcolor{lightlightgrey} 5.6k 
     &\cellcolor{lightlightgrey} code change, review comment 
     &\cellcolor{lightlightgrey} \xmark \\

     Configuring Static Code Analysis Tools (1)
     & - 
     & 1.9k 
     & review comment 
     & \xmark \\ 
     
     \cellcolor{lightlightgrey}Partitioning Static Analysis Warnings (1)
     &\cellcolor{lightlightgrey} ?
     &\cellcolor{lightlightgrey} ?
     &\cellcolor{lightlightgrey} code snippet
     &\cellcolor{lightlightgrey} \\ 
     
     Recommending Reviewers (36)
     & 55 
     & 293.4k 
     & commit, PR, review, review comment
     & 3/36 \\
     
    \cellcolor{lightlightgrey} Visualizing Code Changes (4)
     &\cellcolor{lightlightgrey} 0 
     &\cellcolor{lightlightgrey} 100 
     &\cellcolor{lightlightgrey} commit, diff hunk, PR
     &\cellcolor{lightlightgrey} 2/4\\
     \rulec

    \end{tabular}
    }
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}
\centering
\caption{Code review tasks for which automated solutions have been proposed\vspace{-0.3cm}}
\label{tab:rq2_test}
    {\scriptsize
   \begin{tabular}{ p{7.95cm} | p{1.4cm}| p{1.4cm} | p{1.4cm} | p{1cm}}
    \rulec
  {\bf Task} & {\bf \#1 Metric} & {\bf \#2 Metric} & {\bf \#3 Metric} & {\bf Qualitative} \\  \rulec

    
     %ASSESSING REVIEW QUALITY ---------------------------------------------------------------------------|
      \multicolumn{5}{c}{\bf  Assessing Review Quality} \\ \rulec
     
      Assessing Review Quality through Biometrics (2) 
     & Accuracy
     & F1-score
     & Precision\&Recall
     & \xmark \\
     
     \cellcolor{lightlightgrey}Classifying the Usefulness of Review Comments (4) 
     & Precision\&Recall
     & F1-score 
     & Accuracy
     & \\
     
     Identifying/Improving Review Comments Needing Further Explanations(2) 
     & Accuracy
     & F1-score
     & Correct Explanation
     & 1/2 \\
     \rulec
    
    % CODE CHANGE ANALYSIS ---------------------------------------------------------------------------|
    \multicolumn{5}{c}{\bf Code Change Analysis} \\ \rulec

     \cellcolor{lightlightgrey}Decomposing Tangled Commit (3)
     & Accuracy
     & MAP
     & MRR
     & 2/3\\
     
     Impact Analysis for Code Review (1)
     & Accuracy
     & Recall
     & MAP 
     & \xmark \\
     
     \cellcolor{lightlightgrey}Linking Similar Contributions (2) 
     & 
     &  
     &  
     & \\
     
    Predicting Salient-Class (1)
     & Accuracy
     & Precision\&Recall
     & -
     & \\
    \rulec

     
     % CODE CHANGE CLASSIFICATION ---------------------------------------------------------------------------|
    \multicolumn{5}{c}{\bf Code Change Classification} \\ \rulec
      
     \cellcolor{lightlightgrey}Identifying Impactful Code Changes (2)
     & AUC
     & F1-score
     & Precision\&Recall
     & 1/2\\
    
    Identifying Large-review-effort Code Changes (1) 
     & AUC
     & F1-score
     & Precision\&Recall
     & \\

     \cellcolor{lightlightgrey}Identifying Quickly Reviewable Changes (1) 
     & NDCG
     & -
     & -
     & \\
     
     Predicting Code Changes Approval, Merge, or Need for review (11) 
     & F1-score
     & AUC
     & Precision\&Recall
     & \\
    \rulec

       % CODE CHANGE QUALITY CHECK ---------------------------------------------------------------------------|
     \multicolumn{5}{c}{\bf Code Change Quality Check} \\ \rulec
     
     \cellcolor{lightlightgrey}Checking Design Patterns Consistency (1) 
     & ?
     &  
     &  
     & \\
     
      Generating Review Comments (11) 
     & 
     &  
     &  
     & \\
     
     \cellcolor{lightlightgrey}Identifying Clone Refactoring Opportunities (1) 
     & Accuracy
     & Precision\&Recall 
     &  
     & \\
     
      Predicting Code Defectiveness (2) 
     & F1-score %to check
     & ?
     & ?
     & \\

    \cellcolor{lightlightgrey}Predicting Problematic Code Elements (3) 
     & AUC 
     & F1-score
     & Recall
     & \\
     
     Reviewing Code Formatting Violations (1)
     & Precision
     & Predicion Rate 
     & -
     & \\
     
     \cellcolor{lightlightgrey}Reviewing via Static Analysis (1) 
     & Accuracy
     & -
     & -
     & \\
     \rulec

   % CODE REVIEW SENTIMENT ANALYIS ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Code Review Sentiment Analysis} \\ \rulec
     
      Classifying the Sentiment of Review Comments (1) 
     & Accuracy
     & F1-score
     & Precision\&Recall
     & \\
     
    \cellcolor{lightlightgrey}Identifying “Pushback” Feelings in Reviews (1) 
     & Precision\&Recall
     &  
     &  
     & 1/1 \\
     
     Identifying Toxic/Uncivil Code Review Comments (4)
     & F1-score
     & Precision\&Recall
     & Accuracy
     & \\
     
     \cellcolor{lightlightgrey}Rephrasing Toxic/Uncivil Comments (1) % they also use as metric the score of models to detect the sentiment (e.g. SentiCR, SentiStrength-SE, ...)
     & Incivility Deacrease
     & Length Dissimilarity
     & Semantic Similarity
     & 1/1 \\
     \rulec
     
        % RETRIVIAL OF SIMILAR CR/CC ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Retrieval of Similar CR/CC} \\ \rulec
     
      Augmenting Reviews (8)
     & Accuracy
     & Precision\&Recall % Precision 2, Recall 3
     & MRR % pari merito con BLEU
     & \\
     
     \cellcolor{lightlightgrey}Mining Code Improvement Patterns (1) 
     & Accuracy
     & -
     & -
     & \\
     \rulec
     
     % REVISED CODE GENERATION ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Revised Code Generation} \\ \rulec

     Implementing the Code Change Requested by a Reviewer (11) 
     & Accuracy
     & BLEU
     & CodeBLEU
     & \\
          
      \cellcolor{lightlightgrey}Predicting the Code Output of the Review Process (4) 
     & Accuracy
     & BLEU 
     & Levenshtein Distance
     & \\
      \rulec
     
      % TIME MANAGEMENT ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Time Management} \\ \rulec
   
    Identifying Blocking Actors in Pull Requests (1)
     & MAE % Mean Absolute Error
     & MMRE
     & - 
     & \\
   
     \cellcolor{lightlightgrey}Predicting Pull Request/Code Review Completion Time (5)
     & MAE % Mean Absolute Error
     & MRE % Mean Relative Error
     & ?
     & \\
     
     Prioritizing Review Requests (3)
     & ?
     & ?
     & ?
     & \\
     \rulec
     
      % OTHER ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Other} \\ \rulec
   
     \cellcolor{lightlightgrey}Classifying the Goal of a Review Comment or the Type of Change Triggered by a Comment (3)
     & F1-score
     & Precision\&Recall
     & MCC % Matthew’s Correlation Coefficient
     & 1/3\\

     Configuring Static Code Analysis Tools (1)
     & MAP % both Micro-Averaged Precision and Macro-Averaged Precision
     & MAR % Macro-Averaged Recall
     & Precision\&Recall
     & \\
     
     \cellcolor{lightlightgrey}Partitioning Static Analysis Warnings (1)
     & Review Effort
     & -
     & -
     & \\
     
     Recommending Reviewers (36)
     & MRR % Mean Reciprocal Rank
     & Accuracy
     & Precision\&Recall
     & \\
     
    \cellcolor{lightlightgrey} Visualizing Code Changes (4)
     & -
     & - 
     & -
     & 3/4\\ % 1 paper "We hope to empirically evaluate ... in the future
     \rulec

    \end{tabular}
    }
\end{table}



==> tables/rq3_table_test.tex <==
%!TEX root = ../main.tex

\begin{table}
\centering
\caption{Evaluation of the proposed techniques: Test set size, granularity of the technique, and whether the approach has been deployed to developers\vspace{-0.3cm}}
\label{tab:rq3_test}
    {\scriptsize
   \begin{tabular}{ p{8cm} | p{0.5cm}| p{0.5cm} | p{3.1cm} | p{0.9cm}}
    \rulec
  \multirow{2}{*}{\bf Task} &\multicolumn{2}{c|}{\bf  Test Set Size} &\multirow{2}{*}{\bf Granularity} &  {\bf Approach} \\\cline{2-3}
                                        &       min             &            max              &                                                &  {\bf Deployed} \\ \rulec

    
     %ASSESSING REVIEW QUALITY ---------------------------------------------------------------------------|
      \multicolumn{5}{c}{\bf  Assessing Review Quality} \\ \rulec
     
      Assessing Review Quality through Biometrics (2) 
     & 0.1k %84
     & 0.1k %149 
     & code regions, code review 
     & \xmark \\
     
     \cellcolor{lightlightgrey}Classifying the Usefulness of Review Comments (4) 
     &\cellcolor{lightlightgrey} 0.2k 
     &\cellcolor{lightlightgrey} 1.5k 
     &\cellcolor{lightlightgrey} review comment 
     &\cellcolor{lightlightgrey} 2/3\\ 
     
     Identifying/Improving Review Comments Needing Further Explanations(2) 
     & 0.1k %90
     & 0.7k %744
     & review comment
     & \xmark\\ 
     \rulec
    
    % CODE CHANGE ANALYSIS ---------------------------------------------------------------------------|
    \multicolumn{5}{c}{\bf Code Change Analysis} \\ \rulec

     \cellcolor{lightlightgrey}Decomposing Tangled Commit (3)
     &\cellcolor{lightlightgrey} 0.1k %50 
     &\cellcolor{lightlightgrey} 1k 
     &\cellcolor{lightlightgrey} commit 
     &\cellcolor{lightlightgrey} \xmark\\  
     
     Impact Analysis for Code Review (1)
     & -
     & 8.8k
     & PR
     &  \xmark\\   
     
     \cellcolor{lightlightgrey}Linking Similar Contributions (2) 
     &\cellcolor{lightlightgrey} 7k 
     &\cellcolor{lightlightgrey} 383k 
     &\cellcolor{lightlightgrey} code change, PR 
     &\cellcolor{lightlightgrey} \xmark\\ 
     
    Predicting Salient-Class (1)
    & - 
    & 7.6k
    & commit
    & \xmark\\
    \rulec

     
     % CODE CHANGE CLASSIFICATION ---------------------------------------------------------------------------|
    \multicolumn{5}{c}{\bf Code Change Classification} \\ \rulec
      
     \cellcolor{lightlightgrey}Identifying Impactful Code Changes (2)
     &\cellcolor{lightlightgrey} 0
     &\cellcolor{lightlightgrey} 21.4k
     &\cellcolor{lightlightgrey} commit
     &\cellcolor{lightlightgrey} 1/2\\
     % end row
    
    Identifying Large-review-effort Code Changes (1) 
     & - 
     & 136k 
     & commit
     & 1/1\\

    \cellcolor{lightlightgrey}Identifying Quickly Reviewable Changes (1) 
     &\cellcolor{lightlightgrey} -
     &\cellcolor{lightlightgrey} 100k
     &\cellcolor{lightlightgrey} PR
     &\cellcolor{lightlightgrey} \xmark\\ 
     
     Predicting Code Changes Approval, Merge, or Need for review (11) 
    & 10k
    & 661k %661.4k
    & diff hunk, method, PR
    & \xmark \\
    \rulec

       % CODE CHANGE QUALITY CHECK ---------------------------------------------------------------------------|
     \multicolumn{5}{c}{\bf Code Change Quality Check} \\ \rulec
     
     \cellcolor{lightlightgrey}Checking Design Patterns Consistency (1) 
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} 0.1k %68 
     &\cellcolor{lightlightgrey} file 
     &\cellcolor{lightlightgrey}\xmark \\
     
      Generating Review Comments (11) 
     & 2k 
     & 134k 
     & code change, diff hunk, method
     & \xmark \\
     
     \cellcolor{lightlightgrey}Identifying Clone Refactoring Opportunities (1) 
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} 1.3k %1258 
     &\cellcolor{lightlightgrey} PR 
     &\cellcolor{lightlightgrey} \xmark \\
     
      Predicting Code Defectiveness (2) 
     & 1.4k %1370 
     & 4.7k
     & file, PR
     & 1/2 \\

    \cellcolor{lightlightgrey}Predicting Problematic Code Elements (3) 
     &\cellcolor{lightlightgrey} 2k 
     &\cellcolor{lightlightgrey} 100k
     &\cellcolor{lightlightgrey} code line, file, PR
     &\cellcolor{lightlightgrey} \xmark \\
     
     Reviewing Code Formatting Violations (1)
     & - 
     & 663k
     & file 
     & \xmark \\ 
     
     \cellcolor{lightlightgrey}Reviewing via Static Analysis (1) 
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} 8.7k 
     &\cellcolor{lightlightgrey} PR
     &\cellcolor{lightlightgrey} 1/1 \\
     \rulec

   % CODE REVIEW SENTIMENT ANALYIS ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Code Review Sentiment Analysis} \\ \rulec
     
      Classifying the Sentiment of Review Comments (1) 
     & - 
     & 1.6k 
     & review comment 
     & \xmark \\
     
    \cellcolor{lightlightgrey}Identifying “Pushback” Feelings in Reviews (1) % 2.500 sviluppatori, con 1.317 risposte complete -> non un vero test set
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} code review
     &\cellcolor{lightlightgrey} \xmark\\ 
     
     Identifying Toxic/Uncivil Code Review Comments (4)
     & 3.6k 
     & 19.6k
     & email, review comment, sentence
     & \xmark\\  
     
     \cellcolor{lightlightgrey}Rephrasing Toxic/Uncivil Comments (1)
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} 2.2k 
     &\cellcolor{lightlightgrey} review comment
     &\cellcolor{lightlightgrey} \xmark\\ 
     \rulec
     
        % RETRIVIAL OF SIMILAR CR/CC ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Retrieval of Similar CR/CC} \\ \rulec
     
      \multirow{2}{*}{Augmenting Reviews (8)}
     & \multirow{2}{*}{0.2k} %200 
     & \multirow{2}{*}{150k} 
     & code change, code review, code snippet, diff hunk, review comment
     & \multirow{2}{*}{1/8} \\
     
     \cellcolor{lightlightgrey}Mining Code Improvement Patterns (1) 
     &\cellcolor{lightlightgrey} - 
     &\cellcolor{lightlightgrey} 61.7k 
     &\cellcolor{lightlightgrey} diff hunk 
     &\cellcolor{lightlightgrey} \xmark \\ 
     \rulec
     
     % REVISED CODE GENERATION ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Revised Code Generation} \\ \rulec

     Implementing the Code Change Requested by a Reviewer (11) 
     & 1.7k 
     & 35.6k 
     & code change, diff hunk, method
     & 1/11 \\
          
      \cellcolor{lightlightgrey}Predicting the Code Output of the Review Process (4) 
     &\cellcolor{lightlightgrey} 1.7k 
     &\cellcolor{lightlightgrey} 16.8k 
     &\cellcolor{lightlightgrey} method
     &\cellcolor{lightlightgrey} \xmark \\
      \rulec
     
      % TIME MANAGEMENT ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Time Management} \\ \rulec
   
    Identifying Blocking Actors in Pull Requests (1)
     & - 
     & 2.9k 
     & PR 
     & 1/1 \\
   
     \cellcolor{lightlightgrey}Predicting Pull Request/Code Review Completion Time (5)
     &\cellcolor{lightlightgrey} 2.9k 
     &\cellcolor{lightlightgrey} 2.9k 
     &\cellcolor{lightlightgrey} code change, commit, PR 
     &\cellcolor{lightlightgrey} 2/2 \\
     
     Prioritizing Review Requests (3)
     & 2.9k
     & 661k
     & code change, PR 
     & 2/5 \\ 
     \rulec
     
      % OTHER ---------------------------------------------------------------------------|
   \multicolumn{5}{c}{\bf Other} \\ \rulec
   
     \cellcolor{lightlightgrey}Classifying the Goal of a Review Comment or the Type of Change Triggered by a Comment (3)
     &\cellcolor{lightlightgrey} 1.5k 
     &\cellcolor{lightlightgrey} 5.6k 
     &\cellcolor{lightlightgrey} code change, review comment 
     &\cellcolor{lightlightgrey} \xmark \\

     Configuring Static Code Analysis Tools (1)
     & - 
     & 1.9k 
     & review comment 
     & \xmark \\ 
     
     \cellcolor{lightlightgrey}Partitioning Static Analysis Warnings (1)
     &\cellcolor{lightlightgrey} -
     &\cellcolor{lightlightgrey} 0.1k %95 tasks
     &\cellcolor{lightlightgrey} code snippet
     &\cellcolor{lightlightgrey} \xmark \\ 
     
     Recommending Reviewers (36)
     & 0.1k %47 
     & 293k %293.4k 
     & commit, PR
     & 3/36 \\
     
    \cellcolor{lightlightgrey} Visualizing Code Changes (4)
     &\cellcolor{lightlightgrey} 0 
     &\cellcolor{lightlightgrey} 0.1k %100 
     &\cellcolor{lightlightgrey} commit, diff hunk, PR
     &\cellcolor{lightlightgrey} 2/4\\
     \rulec

    \end{tabular}
    }
\end{table}
